RTMDet: An Empirical Study of Designing Real-Time Object Detectors

In this paper, we aim to design an efficient real-time object detector that exceeds the YOLO series and is easily extensible for many object recognition tasks such as instance segmentation and rotated object detection. To obtain a more efficient model architecture, we explore an architecture that has compatible capacities in the backbone and neck, constructed by a basic building block that consists of large-kernel depth-wise convolutions. We further introduce soft labels when calculating matching costs in the dynamic label assignment to improve accuracy. Together with better training techniques, the resulting object detector, named RTMDet, achieves 52.8% AP on COCO with 300+ FPS on an NVIDIA 3090 GPU, outperforming the current mainstream industrial detectors. RTMDet achieves the best parameter-accuracy trade-off with tiny/small/medium/large/extra-large model sizes for various application scenarios, and obtains new state-of-the-art performance on real-time instance segmentation and rotated object detection. We hope the experimental results can provide new insights into designing versatile real-time object detectors for many object recognition tasks. Code and models are released at https://github.com/open-mmlab/mmdetection/tree/3.x/configs/rtmdet.

==> sections/rebuttal.tex <==
% !TEX root = ../main.tex

\section{Experiments}\label{sec:Experiments}
\subsection{Implementation Details}

% Table:Ablation studies of model architecture
\begin{table*}[t] % 
    \centering
    \caption{\textbf{Ablation studies of model architecture} on COCO \texttt{val2017} set.
    }\label{table:ablation_repr}
    %\vspace{-6pt}
    \centering
    % \footnotesize
    \begin{minipage}[t]{.48\linewidth}
      \centering
      \subcaption{\small{Speed-accuracy trade-off of kernel size}}\label{tab:ablation:kernel_size}
      %\vspace{-3pt}
     \tablestyle{1pt}{1.2}
      \scalebox{0.95}{\begin{tabular}{ c | x{40}x{40}x{40}|x{23}}
        Kernel Size & Params. & GFLOPs & Latency & AP \\
        \shline
        3 & & & & \\
        \ours{5} & & & & \\
        7 & & & & \\
        \end{tabular}}
    \end{minipage}
    \begin{minipage}[t]{.48\linewidth}
      \centering
      \subcaption{\small{Speed-accuracy trade-off of depth and width}}\label{tab:ablation:num_blocks}
      %\vspace{-3pt}
     \tablestyle{1pt}{1.2}
      \scalebox{0.95}{\begin{tabular}{ c | x{40}x{40}x{40}|x{23}}
        Num. Blocks & Params. & GFLOPs & Latency & AP \\
        \shline
        3-9-9-3 & & & & \\
        3-6-6-3 & & & & \\
        3-3-3-3 & & & & \\
        \end{tabular}}
    \end{minipage}
    \begin{minipage}[t]{.48\linewidth}
        \centering
        \subcaption{\small{Design of head}}\label{tab:ablation:head}
        %\vspace{-3pt}
       \tablestyle{1pt}{1.2}
        \scalebox{0.95}{\begin{tabular}{ c | x{40}x{40}x{40}|x{23}}
          Kernel Size & Params. & GFLOPs & Latency & AP \\
          \shline
          shared head & & & & \\
          totally separate & & & & \\
          separate BN & & & & \\
          \end{tabular}}
      \end{minipage}
      \begin{minipage}[t]{.48\linewidth}
        \centering
        \subcaption{\small{Speed-accuracy trade-off of depth and width}}\label{tab:ablation:kernel_size}
        %\vspace{-3pt}
       \tablestyle{1pt}{1.2}
        \scalebox{0.95}{\begin{tabular}{ c | x{40}x{40}x{40}|x{23}}
          Kernel Size & Params. & GFLOPs & Latency & AP \\
          \shline
          shared head & & & & \\
          totally separate & & & & \\
          \ours{separate BN}& & & & \\
          \end{tabular}}
      \end{minipage}
    %\vspace{-18pt}
  \end{table*}
  %##################################################################################################

\subsection{Model Arhitecture}
\paragraph{Large-kernel matters.}

\begin{table}
    \centering
    \caption{\small{Comparison with YOLOX}}\label{tab:ablation:label_assignment}
     %\vspace{-3pt}
    \tablestyle{1pt}{1.2}
     \scalebox{0.95}{\begin{tabular}{ c | x{23} x{23} x{23} | x{23}}
       Kernel size & params & flops & latency & mAP \\
       \shline
       SimOTA &\\
       DSLA  & & &  \\
       \end{tabular}}
    %\vspace{-18pt}
\end{table}


\paragraph{Computation reallocation of multiple feature scales.}
\paragraph{Computation reallocation of backbone and neck.}
\paragraph{Head.}
\subsection{Training Strategy}

\paragraph{Label assignment and losses.}
% Ablation study of label assignment
\begin{table}
    \centering
    \caption{\small{Ablation study of label assignment}}\label{tab:ablation:label_assignment}
    %\vspace{-3pt}
   \tablestyle{1pt}{1.2}
    \scalebox{0.95}{\begin{tabular}{ c x{50} x{55}|x{23}}
      Soft cls. cost & Soft ctr. prior& Loss IoU Cost & mAP \\
      \shline
      $\checkmark$ & & &  \\
      $\checkmark$ &$\checkmark$& & \\
      $\checkmark$ &$\checkmark$ &$\checkmark$ & \\
      \end{tabular}}
%\vspace{-18pt}
\end{table}

% Comparison with other label assignment
\begin{table}
    \centering
    \caption{\small{Comparison with other label assignment}}\label{tab:ablation:label_assignment}
    %\vspace{-3pt}
   \tablestyle{1pt}{1.2}
    \scalebox{0.95}{\begin{tabular}{ c | x{23}| x{23} x{23} x{23}x{23} x{23}}
      Method & AP & AP$_{50}$ & AP$_{70}$ & AP$_{l}$ & AP$_{m}$ & AP$_{l}$ \\
      \shline
      ATSS &\\
      PAA  & & &  \\
      OTA  & & \\
      TOOD & & \\
      Ours & \\
      \end{tabular}}
\end{table}

% Comparison with YOLOX
\begin{table}
\centering
\caption{\small{Comparison with YOLOX}}\label{tab:ablation:label_assignment}
 %\vspace{-3pt}
\tablestyle{1pt}{1.2}
 \scalebox{0.95}{\begin{tabular}{ c | x{23}| x{23} x{23} x{23}x{23} x{23}}
   Method & AP & AP$_{50}$ & AP$_{70}$ & AP$_{l}$ & AP$_{m}$ & AP$_{l}$ \\
   \shline
   SimOTA &\\
   DSLA  & & &  \\
   \end{tabular}}
%\vspace{-18pt}
\end{table}
\paragraph{Data augmentation.}
\paragraph{Optimization strategy.}


\subsection{Step-by-step Results}

\subsection{Generalization Analysis}
\paragraph{Model architecture.}
\paragraph{Training strategy.}

